Evidential Deep Learning for Uncertainty Quantification and Out-of-Distribution Detection in Jet Identification using Deep Neural Networks

Current methods commonly used for uncertainty quantification (UQ) in deep learning (DL) models utilize Bayesian methods which are computationally expensive and time-consuming. In this paper, we provide a detailed study of UQ based on evidential deep learning (EDL) for deep neural network models designed to identify jets in high energy proton-proton collisions at the Large Hadron Collider and explore its utility in anomaly detection. EDL is a DL approach that treats learning as an evidence acquisition process designed to provide confidence (or epistemic uncertainty) about test data. Using publicly available datasets for jet classification benchmarking, we explore hyperparameter optimizations for EDL applied to the challenge of UQ for jet identification. We also investigate how the uncertainty is distributed for each jet class, how this method can be implemented for the detection of anomalies, how the uncertainty compares with Bayesian ensemble methods, and how the uncertainty maps onto latent spaces for the models. Our studies uncover some pitfalls of EDL applied to anomaly detection and a more effective way to quantify uncertainty from EDL as compared with the foundational EDL setup. These studies illustrate a methodological approach to interpreting EDL in jet classification models, providing new insights on how EDL quantifies uncertainty and detects out-of-distribution data which may lead to improved EDL methods for DL models applied to classification tasks.

==> tex-inputs/app-Variants.tex <==
\begin{table}[!ht]
    \centering
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
   Dataset & Training Description & UQ Method & Params & ID Acc & AUROC & AUROC-STD  \\
    \hline
    \multirow{6}{*}{Top tagging dataset} & 
    \multirow{6}{*}{\textit{Baseline}} &
    Ensemble & 968k & \textbf{0.937} & 0.890 & \\
    & &
    MC Dropout & 97k & 0.933 & 0.887 &\\
    & &
    EDL $\lambda_t (0) $ & 97k & \textbf{0.937} & 0.723 & 0.899\\
    & &
    EDL $\lambda_t (0.1) $ & 97k & \textbf{0.937} & 0.902 & 0.903\\
    & &
    EDL $\lambda_t (0.7) $ & 97k & \textbf{0.937} & \textbf{0.904} & \textbf{0.904}\\
    & &
    EDL $\lambda_t (1.0) $ & 97k & \textbf{0.937} & \textbf{0.904} & \textbf{0.904}\\
    \hline
    \end{tabular}
    }
    \caption{In-distribution and UQ performance of the EDL and Ensemble models for different training data in top tagging dataset.} 
    \label{tab:Topdata}
\end{table}

\begin{table}[!ht]
    \centering
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
   Dataset & Training Description & UQ Method & Params & ID Acc & AUROC & AUROC-STD  \\
    \hline
    \multirow{38}{*}{JetNet dataset} & 
    \multirow{10}{*}{\textit{Baseline}} &
    Ensemble & 971k & \textbf{0.806} & 0.772 &\\
    & &
    MC Dropout & 97k & 0.797 & 0.743 & \\
    & &
    EDL $\lambda_t (0) $ & 97k & 0.803 & 0.550 & 0.799\\
    & &
    EDL $\lambda_t (0.1) $ & 97k & 0.799 & 0.811 & 0.813\\
    & &
    EDL $\lambda_t (0.5) $ & 97k & 0.796 & 0.815 & 0.816\\
    & &
    EDL $\lambda_t (0.7) $ & 97k & 0.793 & 0.820 & 0.843\\
    & &
    EDL $\lambda_t (1.0) $ & 97k & 0.790 & 0.822 & 0.823\\
    & &
    EDL-CT $\lambda_t (0.1) $ & 97k & 0.801 & 0.814 & 0.815\\
    & &
    EDL-CT $\lambda_t (0.5) $ & 97k & 0.788 & 0.831 & 0.832\\
    & &
    EDL-CT $\lambda_t (0.7) $ & 97k & 0.776 & \textbf{0.843} & \textbf{0.843}\\
    \cline{2-7}
    &
    \multirow{10}{*}{Skiptop} &
    Ensemble & 970k & \textbf{0.822} & \textbf{0.766} &\\
    & &
    MC Dropout & 97k & 0.810 & 0.656 &\\
    & &
    EDL $\lambda_t (0) $ & 97k & 0.815 & 0.380 & 0.511\\
    & &
    EDL $\lambda_t (0.1) $ & 97k & 0.814 & 0.701 & 0.713\\
    & &
    EDL $\lambda_t (0.5) $ & 97k & 0.815 & 0.754 & 0.754\\
    & &
    EDL $\lambda_t (0.7) $ & 97k & 0.814 & 0.746 & 0.747\\
    & &
    EDL $\lambda_t (1.0) $ & 97k & 0.811 & 0.743 & 0.744\\
    & &
    EDL-CT $\lambda_t (0.1) $ & 97k & 0.814 & 0.724 & 0.729\\
    & &
    EDL-CT $\lambda_t (0.5) $ & 97k & 0.808 & 0.746 & 0.745\\
    & &
    EDL-CT $\lambda_t (0.7) $ & 97k & 0.808 & 0.743 & 0.743\\
    \cline{2-7}
    &
    \multirow{9}{*}{Skipwz} &
    Ensemble & 969k & \textbf{0.824} & 0.741 &\\
    & &
    MC Dropout & 97k & 0.817 & 0.717 &\\
    & &
    EDL $\lambda_t (0) $ & 97k & 0.818 & \textbf{0.824}& 0.753\\
    & &
    EDL $\lambda_t (0.1) $ & 97k & 0.816 & 0.701 & 0.697\\
    & &
    EDL $\lambda_t (0.6) $ & 97k & 0.814 & 0.690 & 0.690\\
    & &
    EDL $\lambda_t (1.0) $ & 97k & 0.815 & 0.666 & 0.666\\
    & &
    EDL-CT $\lambda_t (0.1) $ & 97k & 0.817 & 0.676 & 0.676\\
    & &
    EDL-CT $\lambda_t (0.5) $ & 97k & 0.816 & 0.681 & 0.680\\
    & &
    EDL-CT $\lambda_t (0.7) $ & 97k & 0.816 & 0.692 & 0.691\\
    \cline{2-7}
    &
    \multirow{9}{*}{Skiptwz} &
    Ensemble & 968k & 0.824 & \textbf{0.741} &\\
    & &
    MC Dropout & 97k & 0.833 & 0.693 &\\
    & &
    EDL $\lambda_t (0) $ & 97k & \textbf{0.837} & 0.386 & 0.614\\
    & &
    EDL $\lambda_t (0.1) $ & 97k & 0.836 & 0.713 & 0.709 \\
    & &
    EDL $\lambda_t (0.6) $ & 97k & \textbf{0.837} & 0.714 & 0.687\\
    & &
    EDL $\lambda_t (1.0) $ & 97k & 0.836 & 0.690 & 0.690\\
    & &
    EDL-CT $\lambda_t (0.1) $ & 97k & 0.836 & 0.635 & 0.681\\
    & &
    EDL-CT $\lambda_t (0.5) $ & 97k & 0.835 & 0.694 & 0.694\\
    & &
    EDL-CT $\lambda_t (0.7) $ & 97k & 0.835 & 0.697 & 0.697\\
    \hline
    \end{tabular}
    }
    \caption{In-distribution and UQ performance of the EDL and Ensemble models for different training data in JetNet dataset. } 
    \label{tab:JetNet}
\end{table}

\begin{table}[!ht]
    \centering
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
   Dataset & Training Description & UQ Method & Params & ID Acc & AUROC & AUROC-STD\\
    \hline
    \multirow{25}{*}{JetClass dataset} & 
    \multirow{5}{*}{\textit{Baseline}} &
    Ensemble & 994k & \textbf{0.805} & 0.782 &\\
    & &
    MC Dropout & 99k & 0.793 & 0.745 &\\
    & &
    EDL $\lambda_t (0) $ & 99k & 0.794 & 0.602 & 0.816\\
    & &
    EDL $\lambda_t (0.1) $ & 99k & 0.792 & 0.842  & 0.843\\
    & &
    EDL $\lambda_t (1.0) $ & 99k & 0.776 & \textbf{0.847} & \textbf{0.847}\\
    \cline{2-7}
    &
    \multirow{5}{*}{Skiptop} &
    Ensemble & 992k & \textbf{0.782} & \textbf{0.623} &\\
    & &
    MC Dropout & 99k & 0.750 & 0.615 &\\
    & &
    EDL $\lambda_t (0) $ & 99k & 0.773 & 0.483 & 0.527\\
    & &
    EDL $\lambda_t (0.1) $ & 99k & 0.763 & 0.509 & 0.507\\
    & &
    EDL $\lambda_t (1.0) $ & 99k & 0.749 & 0.505 & 0.506\\
    \cline{2-7}
    &
    \multirow{5}{*}{Skipwz} &
    Ensemble & 992k & \textbf{0.862} & 0.754 &\\
    & &
    MC Dropout & 99k & 0.777 & 0.730 &\\
    & &
    EDL $\lambda_t (0) $ & 99k & 0.845 & 0.788 & \textbf{0.819}\\
    & &
    EDL $\lambda_t (0.1) $ & 99k & 0.847 & 0.771 & 0.770\\
    & &
    EDL $\lambda_t (1.0) $ & 99k & 0.848 & 0.776 & 0.776\\
    \cline{2-7}
    &
    \multirow{5}{*}{Skiptwz} &
    Ensemble & 990k & \textbf{0.845} & \textbf{0.725} &\\
    & &
    MC Dropout & 99k & 0.755 & 0.638 &\\
    & &
    EDL $\lambda_t (0) $ & 99k & 0.837 & 0.664 &  0.681\\
    & &
    EDL $\lambda_t (0.1) $ & 99k & 0.833 & 0.650 & 0.648\\
    & &
    EDL $\lambda_t (1.0) $ & 99k & 0.833 & 0.659 & 0.658\\
    \cline{2-7}
    &
    \multirow{5}{*}{Skiph} &
    Ensemble & 989k & \textbf{0.830} & 0.710 &\\
    & &
    MC Dropout & 99k & 0.811 & 0.739 &\\
    & &
    EDL $\lambda_t (0) $ & 99k & 0.828 & \textbf{0.797} & 0.756\\
    & &
    EDL $\lambda_t (0.1) $ & 99k & \textbf{0.830} & 0.689 &0.685\\
    & &
    EDL $\lambda_t (1.0) $ & 99k & 0.827 & 0.691 & 0.690\\
    \hline
    \end{tabular}
    }
    \caption{In-distribution and UQ performance of the EDL and Ensemble models for different training data in JetClass dataset.} 
    \label{tab:JetClass}
\end{table}

==> tex-inputs/app-baseline.tex <==
\begin{table}[!ht]
    \centering
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
   Dataset & Model & Params & Accuracy & AUROC & AUROC-STD  \\
    \hline
    \multirow{6}{*}{Top tagging} & 
    Ensemble & 968k & 0.937 & 0.890 & \\
    & 
    MC Dropout & 97k & 0.933 & 0.887 &\\
    &
    EDL $\lambda_t (0) $ & 97k & 0.937 & 0.723 & 0.899\\
    &
    EDL $\lambda_t (0.1) $ & 97k & 0.937 & 0.902 & 0.903\\
    &
    EDL $\lambda_t (0.7) $ & 97k & 0.937 & 0.904 & \textbf{0.904}\\
    &
    EDL $\lambda_t (1.0) $ & 97k & \textbf{0.937} & \textbf{0.904} & \textbf{0.904}\\
    \hline
    \multirow{10}{*}{JetNet} & 
    Ensemble & 971k & 0.806 & 0.772 &\\
    &
    MC Dropout & 97k & 0.797 & 0.743 & \\
    &
    EDL $\lambda_t (0) $ & 97k & 0.803 & 0.550 & 0.799\\
    &
    EDL $\lambda_t (0.1) $ & 97k & 0.799 & 0.811 & 0.813\\
    &
    EDL $\lambda_t (0.5) $ & 97k & 0.796 & 0.815 & 0.816\\
    &
    EDL $\lambda_t (0.7) $ & 97k & 0.793 & 0.820 & 0.843\\
    &
    EDL $\lambda_t (1.0) $ & 97k & 0.790 & 0.822 & 0.823\\
    &
    EDL-CT $\lambda_t (0.1) $ & 97k & \textbf{0.801} & \textbf{0.814} & \textbf{0.815}\\
    &
    EDL-CT $\lambda_t (0.5) $ & 97k & 0.788 & 0.831 & 0.832\\
    &
    EDL-CT $\lambda_t (0.7) $ & 97k & 0.776 & 0.843 & 0.843\\
    \hline
    \multirow{5}{*}{JetClass} & 
    Ensemble & 994k & 0.805 & 0.782 &\\
    &
    MC Dropout & 99k & 0.793 & 0.745 &\\
    &
    EDL $\lambda_t (0) $ & 99k & 0.794 & 0.602 & 0.816\\
    &
    EDL $\lambda_t (0.1) $ & 99k & \textbf{0.792} & \textbf{0.842}  & \textbf{0.843}\\
    &
    EDL $\lambda_t (1.0) $ & 99k & 0.776 & 0.847 & 0.847\\
    \hline
    \end{tabular}
    }
    \caption{Accuracy and AUROC of the EDL and Ensemble models for different baseline datasets. The rows marked in \textbf{bold} represent the best-performing EDL model for the corresponding dataset.} 
    \label{tab:baseline-old}
\end{table}


\begin{table}[!ht]
 \centering
 \resizebox{0.99\textwidth}{!}{
 \begin{tabular}{|l||c|c|c||c|c|c||c|c|c|}
    \hline
   & \multicolumn{3}{c||}{\topdata} & \multicolumn{3}{c||}{\jetnet} & \multicolumn{3}{c|}{\jetclass} \\ \hline \hline
    \textbf{Model} & Acc & AUC & STD & Acc & AUC & STD & Acc & AUC & STD  \\ \hline
    Ensemble & 0.937 & 0.890 & - & 0.806 & 0.772 & - & 0.805 & 0.782 & -  \\ \hline
    MC Dropout & 0.933 & 0.887 & - & 0.797 & 0.743 & - & 0.793 & 0.745 & -  \\ \hline \hline
    EDL $\lambda_t (0)$ & 0.937 & 0.723 & 0.899 & \textbf{0.803} & 0.550 & 0.799 & \textbf{0.794} & 0.602 & 0.816 \\
    EDL $\lambda_t (0.1)$ & 0.937 & 0.902 & 0.903 & 0.799 & 0.811 & 0.813 & 0.792 & 0.842 & 0.843 \\
    EDL $\lambda_t (0.5)$ & - & - & - & 0.796 & 0.815 & 0.816 & - & - & - \\
    EDL $\lambda_t (0.7)$ & 0.937 & 0.904 & 0.904 & 0.793 & 0.820 & 0.843 & - & - & - \\
    EDL $\lambda_t (1.0)$ & \textbf{0.937} & \textbf{0.904} & \textbf{0.904} & 0.790 & 0.822 & 0.823 & 0.776 & \textbf{0.847} & \textbf{0.847} \\
    EDL-CT $\lambda_t^{\texttt{CT}} (0.1)$ & - & - & - & 0.801 & 0.814 & 0.815 & - & - & - \\
    EDL-CT $\lambda_t^{\texttt{CT}} (0.5)$ & - & - & - & 0.788 & 0.831 & 0.832 & - & - & - \\
    EDL-CT $\lambda_t^{\texttt{CT}} (0.7)$ & - & - & - & 0.776 & \textbf{0.843} & \textbf{0.843} & - & - & - \\
    \hline
  \end{tabular}
  }
  \caption{ID Accuracy (Acc), AUROC (AUC), and AUROC-STD (STD) of the EDL and Ensemble methods on \topdata, \jetnet, and \jetclass datasets. Within \topdata and \jetnet models, the Ensemble model has 970k parameters, while all other models have 97k parameters. The \jetclass Ensemble model has 994k parameters, while all other \jetclass models have 99k parameters. For each dataset, the entries marked in \textbf{bold} represent the EDL model with the highest central value for the corresponding metric. These measurements have uncertainties of $\mathcal{O}(0.001)$.}
  \label{tab:baseline}
\end{table}

% \begin{table}[!ht]
%     \centering
%     \resizebox{0.9\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%    Dataset & Training Description & UQ Method & Params & ID Acc & AUROC & AUROC-STD  \\
%     \hline
%     \multirow{38}{*}{JetNet dataset} & 
%     \multirow{10}{*}{\textit{Baseline}} &
%     Ensemble & 971k & \textbf{0.806} & 0.772 &\\
%     & &
%     MC Dropout & 97k & 0.797 & 0.743 & \\
%     & &
%     EDL $\lambda_t (0) $ & 97k & 0.803 & 0.550 & 0.799\\
%     & &
%     EDL $\lambda_t (0.1) $ & 97k & 0.799 & 0.811 & 0.813\\
%     & &
%     EDL $\lambda_t (0.5) $ & 97k & 0.796 & 0.815 & 0.816\\
%     & &
%     EDL $\lambda_t (0.7) $ & 97k & 0.793 & 0.820 & 0.843\\
%     & &
%     EDL $\lambda_t (1.0) $ & 97k & 0.790 & 0.822 & 0.823\\
%     & &
%     EDL-CT $\lambda_t (0.1) $ & 97k & 0.801 & 0.814 & 0.815\\
%     & &
%     EDL-CT $\lambda_t (0.5) $ & 97k & 0.788 & 0.831 & 0.832\\
%     & &
%     EDL-CT $\lambda_t (0.7) $ & 97k & 0.776 & \textbf{0.843} & \textbf{0.843}\\
%     \cline{2-7}
%     &
%     \multirow{10}{*}{Skiptop} &
%     Ensemble & 970k & \textbf{0.822} & \textbf{0.766} &\\
%     & &
%     MC Dropout & 97k & 0.810 & 0.656 &\\
%     & &
%     EDL $\lambda_t (0) $ & 97k & 0.815 & 0.380 & 0.511\\
%     & &
%     EDL $\lambda_t (0.1) $ & 97k & 0.814 & 0.701 & 0.713\\
%     & &
%     EDL $\lambda_t (0.5) $ & 97k & 0.815 & 0.754 & 0.754\\
%     & &
%     EDL $\lambda_t (0.7) $ & 97k & 0.814 & 0.746 & 0.747\\
%     & &
%     EDL $\lambda_t (1.0) $ & 97k & 0.811 & 0.743 & 0.744\\
%     & &
%     EDL-CT $\lambda_t (0.1) $ & 97k & 0.814 & 0.724 & 0.729\\
%     & &
%     EDL-CT $\lambda_t (0.5) $ & 97k & 0.808 & 0.746 & 0.745\\
%     & &
%     EDL-CT $\lambda_t (0.7) $ & 97k & 0.808 & 0.743 & 0.743\\
%     \cline{2-7}
%     &
%     \multirow{9}{*}{Skipwz} &
%     Ensemble & 969k & \textbf{0.824} & 0.741 &\\
%     & &
%     MC Dropout & 97k & 0.817 & 0.717 &\\
%     & &
%     EDL $\lambda_t (0) $ & 97k & 0.818 & \textbf{0.824}& 0.753\\
%     & &
%     EDL $\lambda_t (0.1) $ & 97k & 0.816 & 0.701 & 0.697\\
%     & &
%     EDL $\lambda_t (0.6) $ & 97k & 0.814 & 0.690 & 0.690\\
%     & &
%     EDL $\lambda_t (1.0) $ & 97k & 0.815 & 0.666 & 0.666\\
%     & &
%     EDL-CT $\lambda_t (0.1) $ & 97k & 0.817 & 0.676 & 0.676\\
%     & &
%     EDL-CT $\lambda_t (0.5) $ & 97k & 0.816 & 0.681 & 0.680\\
%     & &
%     EDL-CT $\lambda_t (0.7) $ & 97k & 0.816 & 0.692 & 0.691\\
%     \cline{2-7}
%     &
%     \multirow{9}{*}{Skiptwz} &
%     Ensemble & 968k & 0.824 & \textbf{0.741} &\\
%     & &
%     MC Dropout & 97k & 0.833 & 0.693 &\\
%     & &
%     EDL $\lambda_t (0) $ & 97k & \textbf{0.837} & 0.386 & 0.614\\
%     & &
%     EDL $\lambda_t (0.1) $ & 97k & 0.836 & 0.713 & 0.709 \\
%     & &
%     EDL $\lambda_t (0.6) $ & 97k & \textbf{0.837} & 0.714 & 0.687\\
%     & &
%     EDL $\lambda_t (1.0) $ & 97k & 0.836 & 0.690 & 0.690\\
%     & &
%     EDL-CT $\lambda_t (0.1) $ & 97k & 0.836 & 0.635 & 0.681\\
%     & &
%     EDL-CT $\lambda_t (0.5) $ & 97k & 0.835 & 0.694 & 0.694\\
%     & &
%     EDL-CT $\lambda_t (0.7) $ & 97k & 0.835 & 0.697 & 0.697\\
%     \hline
%     \end{tabular}
%     }
%     \caption{In-distribution and UQ performance of the EDL and Ensemble models for different training data in JetNet dataset. } 
%     \label{tab:JetNet}
% \end{table}

% \begin{table}[!ht]
%     \centering
%     \resizebox{0.9\textwidth}{!}{
%     \begin{tabular}{|c|c|c|c|c|c|c|}
%     \hline
%    Dataset & Training Description & UQ Method & Params & ID Acc & AUROC & AUROC-STD\\
%     \hline
%     \multirow{25}{*}{JetClass dataset} & 
%     \multirow{5}{*}{\textit{Baseline}} &
%     Ensemble & 994k & \textbf{0.805} & 0.782 &\\
%     & &
%     MC Dropout & 99k & 0.793 & 0.745 &\\
%     & &
%     EDL $\lambda_t (0) $ & 99k & 0.794 & 0.602 & 0.816\\
%     & &
%     EDL $\lambda_t (0.1) $ & 99k & 0.792 & 0.842  & 0.843\\
%     & &
%     EDL $\lambda_t (1.0) $ & 99k & 0.776 & \textbf{0.847} & \textbf{0.847}\\
%     \cline{2-7}
%     &
%     \multirow{5}{*}{Skiptop} &
%     Ensemble & 992k & \textbf{0.782} & \textbf{0.623} &\\
%     & &
%     MC Dropout & 99k & 0.750 & 0.615 &\\
%     & &
%     EDL $\lambda_t (0) $ & 99k & 0.773 & 0.483 & 0.527\\
%     & &
%     EDL $\lambda_t (0.1) $ & 99k & 0.763 & 0.509 & 0.507\\
%     & &
%     EDL $\lambda_t (1.0) $ & 99k & 0.749 & 0.505 & 0.506\\
%     \cline{2-7}
%     &
%     \multirow{5}{*}{Skipwz} &
%     Ensemble & 992k & \textbf{0.862} & 0.754 &\\
%     & &
%     MC Dropout & 99k & 0.777 & 0.730 &\\
%     & &
%     EDL $\lambda_t (0) $ & 99k & 0.845 & 0.788 & \textbf{0.819}\\
%     & &
%     EDL $\lambda_t (0.1) $ & 99k & 0.847 & 0.771 & 0.770\\
%     & &
%     EDL $\lambda_t (1.0) $ & 99k & 0.848 & 0.776 & 0.776\\
%     \cline{2-7}
%     &
%     \multirow{5}{*}{Skiptwz} &
%     Ensemble & 990k & \textbf{0.845} & \textbf{0.725} &\\
%     & &
%     MC Dropout & 99k & 0.755 & 0.638 &\\
%     & &
%     EDL $\lambda_t (0) $ & 99k & 0.837 & 0.664 &  0.681\\
%     & &
%     EDL $\lambda_t (0.1) $ & 99k & 0.833 & 0.650 & 0.648\\
%     & &
%     EDL $\lambda_t (1.0) $ & 99k & 0.833 & 0.659 & 0.658\\
%     \cline{2-7}
%     &
%     \multirow{5}{*}{Skiph} &
%     Ensemble & 989k & \textbf{0.830} & 0.710 &\\
%     & &
%     MC Dropout & 99k & 0.811 & 0.739 &\\
%     & &
%     EDL $\lambda_t (0) $ & 99k & 0.828 & \textbf{0.797} & 0.756\\
%     & &
%     EDL $\lambda_t (0.1) $ & 99k & \textbf{0.830} & 0.689 &0.685\\
%     & &
%     EDL $\lambda_t (1.0) $ & 99k & 0.827 & 0.691 & 0.690\\
%     \hline
%     \end{tabular}
%     }
%     \caption{In-distribution and UQ performance of the EDL and Ensemble models for different training data in JetClass dataset.} 
%     \label{tab:JetClass}
% \end{table}

==> tex-inputs/app-skipx-jetnet.tex <==
\begin{table}[!ht]
    \centering
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|}
    \hline
   Dataset & Model & Params & ID Acc & AUROC & AUROC-STD  \\
    \hline
    \multirow{10}{*}{Skiptop} &
    Ensemble & 970k & \textbf{0.822} & \textbf{0.766} &\\
    &
    MC Dropout & 97k & 0.810 & 0.656 &\\
    &
    EDL $\lambda_t (0) $ & 97k & 0.815 & 0.380 & 0.511\\
    &
    EDL $\lambda_t (0.1) $ & 97k & 0.814 & 0.701 & 0.713\\
    &
    EDL $\lambda_t (0.5) $ & 97k & 0.815 & 0.754 & 0.754\\
    &
    EDL $\lambda_t (0.7) $ & 97k & 0.814 & 0.746 & 0.747\\
    &
    EDL $\lambda_t (1.0) $ & 97k & 0.811 & 0.743 & 0.744\\
    &
    EDL-CT $\lambda_t (0.1) $ & 97k & 0.814 & 0.724 & 0.729\\
    &
    EDL-CT $\lambda_t (0.5) $ & 97k & 0.808 & 0.746 & 0.745\\
    &
    EDL-CT $\lambda_t (0.7) $ & 97k & 0.808 & 0.743 & 0.743\\
    \hline
    \multirow{9}{*}{Skipwz} &
    Ensemble & 969k & \textbf{0.824} & 0.741 &\\
    &
    MC Dropout & 97k & 0.817 & 0.717 &\\
    &
    EDL $\lambda_t (0) $ & 97k & 0.818 & \textbf{0.824}& 0.753\\
    &
    EDL $\lambda_t (0.1) $ & 97k & 0.816 & 0.701 & 0.697\\
    &
    EDL $\lambda_t (0.6) $ & 97k & 0.814 & 0.690 & 0.690\\
    &
    EDL $\lambda_t (1.0) $ & 97k & 0.815 & 0.666 & 0.666\\
    &
    EDL-CT $\lambda_t (0.1) $ & 97k & 0.817 & 0.676 & 0.676\\
    &
    EDL-CT $\lambda_t (0.5) $ & 97k & 0.816 & 0.681 & 0.680\\
    &
    EDL-CT $\lambda_t (0.7) $ & 97k & 0.816 & 0.692 & 0.691\\
    \hline
    \multirow{9}{*}{Skiptwz} &
    Ensemble & 968k & 0.824 & \textbf{0.741} &\\
    &
    MC Dropout & 97k & 0.833 & 0.693 &\\
    &
    EDL $\lambda_t (0) $ & 97k & \textbf{0.837} & 0.386 & 0.614\\
    &
    EDL $\lambda_t (0.1) $ & 97k & 0.836 & 0.713 & 0.709 \\
    &
    EDL $\lambda_t (0.6) $ & 97k & \textbf{0.837} & 0.714 & 0.687\\
    &
    EDL $\lambda_t (1.0) $ & 97k & 0.836 & 0.690 & 0.690\\
    &
    EDL-CT $\lambda_t (0.1) $ & 97k & 0.836 & 0.635 & 0.681\\
    &
    EDL-CT $\lambda_t (0.5) $ & 97k & 0.835 & 0.694 & 0.694\\
    &
    EDL-CT $\lambda_t (0.7) $ & 97k & 0.835 & 0.697 & 0.697\\
    \hline
    \end{tabular}
    }
    \caption{ID Accuracy and AUROC for OOD jet detection using the EDL and Ensemble methods for variants of the JetNet dataset.} 
    \label{tab:skipx-jetnet-old}
\end{table}

\begin{table}[!ht]
 \centering
 \resizebox{0.99\textwidth}{!}{
 \begin{tabular}{|l||c|c|c||c|c|c||c|c|c|}
    \hline
   & \multicolumn{3}{c||}{\skiptop} & \multicolumn{3}{c||}{\skipwz} & \multicolumn{3}{c|}{\skiptwz} \\ \hline \hline
    \textbf{Model} & Acc & AUC & STD & Acc & AUC & STD & Acc & AUC & STD  \\ \hline
    Ensemble & 0.822 & 0.766 & - & 0.824 & 0.741 & - & 0.824 & 0.741 & -  \\ \hline
    MC Dropout & 0.810 & 0.656 & - & 0.817 & 0.717 & - & 0.833 & 0.693 & -  \\ \hline \hline
    EDL $\lambda_t (0)$ & \textbf{0.815} & 0.380 & 0.511 & \textbf{0.818} & \textbf{0.824} & \textbf{0.753} & \textbf{0.837} & 0.386 & 0.614 \\ \hline
    EDL $\lambda_t (0.1)$ & 0.814 & 0.701 & 0.713 & 0.816 & 0.701 & 0.697 & 0.836 & 0.713 & \textbf{0.709} \\ \hline
    EDL $\lambda_t (0.5)$ & \textbf{0.815} & 0.754 & 0.754 & 0.816 & 0.697 & 0.696 & 0.833 & 0.682 & 0.682 \\ \hline
    EDL $\lambda_t (0.6)$ & 0.813 & \textbf{0.756} & \textbf{0.757} & 0.814 & 0.690 & 0.690 & \textbf{0.837} & \textbf{0.714} & 0.687 \\ \hline
    EDL $\lambda_t (1.0)$ & 0.811 & 0.743 & 0.744 & 0.815 & 0.666 & 0.666 & 0.836 & 0.690 & 0.690 \\ \hline
    EDL-CT $\lambda_t^{\texttt{CT}} (0.1)$ & 0.814 & 0.724 & 0.729 & 0.817 & 0.676 & 0.676 & 0.836 & 0.635 & 0.681 \\ \hline
    EDL-CT $\lambda_t^{\texttt{CT}} (0.5)$ & 0.808 & 0.746 & 0.745 & 0.816 & 0.681 & 0.680 & 0.835 & 0.694 & 0.694 \\ \hline
    EDL-CT $\lambda_t^{\texttt{CT}} (0.7)$ & 0.808 & 0.743 & 0.743 & 0.816 & 0.692 & 0.691 & 0.835 & 0.697 & 0.697 \\ \hline 
  \end{tabular}
  }
  \caption{ID Accuracy (Acc),  AUROC (AUC), and AUROC-STD (STD) of the EDL and Ensemble methods on variants of \JetNet: \skiptop, \skipwz, \skiptwz. The Ensemble model has 970k parameters, while all other models have 97k parameters. For each of the \JetNet variants, the entries marked in \textbf{bold} represent the EDL model with the highest central value for the corresponding metric. These measurements have uncertainties of $\mathcal{O}(0.001)$.}
  \label{tab:skipx-jetnet}
\end{table}
  

==> tex-inputs/jetclass_ad.tex <==
\subsection{JetClass dataset}

To further illustrate the capabilities of JetClass models under anomaly detection, we display 4 different training methods: skiptop, skiptwz, skiptwz, and skiph. Their ID and OOD data are described in Table~\ref{tab:JetClassB}, and their performance is outlined in Table~\ref{tab:JetClass}. As said previously, the classes of the dataset and their indices are: $ q/g$ (0), $H \to b \bar{b}$ (1), $H \to c \bar{c}$ (2), $H \to gg$ (3), $H \to 4 q$ (4), $H \to \ell v q q'$ (5), $Z \to q \bar{q}$ (6), $W \to q q'$ (7), $t \to bqq'$ (8), $t \to b \ell v$ (9). The models are evaluated based on the same metrics of the baseline models as stated in Section~\ref{sec:metrics}. 


When we skip top quarks $t$, the anomaly detection is fairly inaccurate for EDL networks because the AUROC and AUROC-STD for skiptop JetClass EDL networks are all below 0.6 in Table~\ref{tab:JetClass}. To examine why this occurs, we plot the uncertainty distributions for each label and prediction in Figure~\ref{fig:jetclass_skiptop}(a)-(b) for EDL $\lambda_t (1.0)$ both without and with D-STD uncertainty. In both cases, the OOD jet $t \to b \ell v$ is often predicted as $H \to \ell v q q'$ with low uncertainties, which drives down AUROC and AUROC-STD. Since $H \to \ell v q q'$ is the only trained jet containing a lepton, the model believes that any jets containing leptons must be $H \to \ell v q q'$ with low uncertainty. Due to the high uncertainties of misclassified jets and low uncertainties of $t \to b \ell v$, there is a significant bimodal distribution in Figure~\ref{fig:jetclass_skiptop}(c)-(f). The uncertainty and maximum probability follow a very straight line, which is not optimal for anomaly detection where the maximum probability and uncertainty shouldn't be correlated. The best performing skiptop JetClass EDL model is EDL $\lambda_t (0)$ with D-STD uncertainty, as displayed in Figure~\ref{fig:jetclass_skiptop}(i)-(j). As opposed to the EDl $\lambda_t (0)$ model with normal uncertainty in Figure~\ref{fig:jetclass_skiptop}(g)-(h), D-STD uncertainty helps the anomaly detection performance for EDL models with $\zeta = 0$ and may slightly hurt the performance of EDL models with non-zero $\zeta$. As opposed to EDL $\lambda_t (1.0)$, the EDL $\lambda_t (0)$ model doesn't have many high-uncertainty ID misclassified jets that result in false positives. However, it also continues to suffer from overall low uncertainty OOD jets because it was trained with $\zeta=0$, which doesn't include the KL-divergence term to increase uncertainty. But with D-STD, the uncertainty range increases, and the OOD uncertainties increase slightly. The maximum probability and uncertainty are also not highly correlated, which creates higher AUROC-STD.


\begin{figure}[!h]

\centering
    
    \subfloat[]{
    \includegraphics[width=0.5\textwidth]{figures/jetclass/skiptop/1.0/labels_preds_unc_total.pdf}
    \label{fig:jetclass_1.0_skiptop_lpu}
    }
    \subfloat[]{
    \includegraphics[width=0.5\textwidth]{figures/jetclass/skiptop/1.0_std/labels_preds_unc_total.pdf}
    \label{fig:jetclass_1.0_std_skiptop_lpu}
    }
% 0.23, 0.27

    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiptop/1.0/unc_separate_log.pdf}
        \label{fig:jetclass_1.0_skiptop_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiptop/1.0/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_1.0_skiptop_up}
    }
    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiptop/1.0_std/unc_separate_log.pdf}
        \label{fig:jetclass_1.0_std_skiptop_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiptop/1.0_std/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_1.0_std_skiptop_up}
    }

    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiptop/0/unc_separate_log.pdf}
        \label{fig:jetclass_0_skiptop_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiptop/0/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_0_skiptop_up}
    }
    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiptop/0_std/unc_separate_log.pdf}
        \label{fig:jetclass_0_std_skiptop_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiptop/0_std/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_0_std_skiptop_up}
    }
    
    
    \caption{\protect\subref{fig:jetclass_1.0_skiptop_lpu},\protect\subref{fig:jetclass_1.0_std_skiptop_lpu} 2D histogram of the predicted label plus the uncertainty versus label, \protect\subref{fig:jetclass_1.0_skiptop_us},\protect\subref{fig:jetclass_1.0_std_skiptop_us} uncertainty distribution, separated by correctly and incorrectly classified jets, and \protect\subref{fig:jetclass_1.0_skiptop_up},\protect\subref{fig:jetclass_1.0_std_skiptop_up} logarithmic 2D histogram of maximum probability versus uncertainty for, respectively, skiptop JetClass EDL $\lambda_t (1.0) $ without and with D-STD uncertainty.
    \protect\subref{fig:jetclass_0_skiptop_us},\protect\subref{fig:jetclass_0_std_skiptop_us} uncertainty distribution, separated by correctly and incorrectly classified jets, and \protect\subref{fig:jetclass_0_skiptop_up},\protect\subref{fig:jetclass_0_std_skiptop_up} logarithmic 2D histogram of maximum probability versus uncertainty for, respectively, skiptop JetClass EDL $\lambda_t (0) $ without and with D-STD uncertainty.
    }
    \label{fig:jetclass_skiptop}
\end{figure}

In this skipwz case, the OOD boson jets don't hold decay into any unique particles that the model hasn't trained on, like leptons. As a result, as shown in Figure~\ref{fig:jetclass_skipwz}, there are very few low-uncertainty OOD jets and the AUROC in Table~\ref{tab:JetClass} are all above 0.7. As we increase the $\zeta$ parameter, the acuraccy stays consistent. The highest AUROC comes from EDL $\lamdba_t (0)$, which performs much better than EDL models with non-zero $\zeta$. The D-STD significantly helps the AUROC of EDL $\lamdba_t (0)$, improving the performance by 0.03. Again, the D-STD has neglible or worse performance on non-zero $\zeta$. We can examine why EDL models with high $\zeta$ underperform in Figure~\ref{fig:jetclass_skipwz}(c)-(f). The primary factor with high $\zeta$ EDL models seems to be the significant number of false positives due to high-uncertainty ID jets. Although EDL $\lambda_t (0)$ doesn't have many high-uncertainty OOD jets, the model quantifies much fewer false positives, which overall increases the AUROC. The D-STD uncertainty helps to increase the uncertainty range significantly and makes OOD jets have overall higher uncertainties. Again, the less linear representation between uncertainty and maximum probability makes it more optimal for anomaly detection, since the confidence of the prediction isn't associated with it being anomalous.


\begin{figure}[!h]

\centering
    
    \subfloat[]{
    \includegraphics[width=0.5\textwidth]{figures/jetclass/skipwz/1.0/labels_preds_unc_total.pdf}
    \label{fig:jetclass_1.0_skipwz_lpu}
    }
    \subfloat[]{
    \includegraphics[width=0.5\textwidth]{figures/jetclass/skipwz/1.0_std/labels_preds_unc_total.pdf}
    \label{fig:jetclass_1.0_std_skipwz_lpu}
    }
% 0.23, 0.27

    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skipwz/1.0/unc_separate_log.pdf}
        \label{fig:jetclass_1.0_skipwz_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skipwz/1.0/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_1.0_skipwz_up}
    }
    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skipwz/1.0_std/unc_separate_log.pdf}
        \label{fig:jetclass_1.0_std_skipwz_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skipwz/1.0_std/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_1.0_std_skipwz_up}
    }

    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skipwz/0/unc_separate_log.pdf}
        \label{fig:jetclass_0_skipwz_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skipwz/0/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_0_skipwz_up}
    }
    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skipwz/0_std/unc_separate_log.pdf}
        \label{fig:jetclass_0_std_skipwz_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skipwz/0_std/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_0_std_skipwz_up}
    }
    
    
    \caption{\protect\subref{fig:jetclass_1.0_skipwz_lpu},\protect\subref{fig:jetclass_1.0_std_skipwz_lpu} 2D histogram of the predicted label plus the uncertainty versus label, \protect\subref{fig:jetclass_1.0_skipwz_us},\protect\subref{fig:jetclass_1.0_std_skipwz_us} uncertainty distribution, separated by correctly and incorrectly classified jets, and \protect\subref{fig:jetclass_1.0_skipwz_up},\protect\subref{fig:jetclass_1.0_std_skipwz_up} logarithmic 2D histogram of maximum probability versus uncertainty for, respectively, skipwz JetClass EDL $\lambda_t (1.0) $ without and with D-STD uncertainty.
    \protect\subref{fig:jetclass_0_skipwz_us},\protect\subref{fig:jetclass_0_std_skipwz_us} uncertainty distribution, separated by correctly and incorrectly classified jets, and \protect\subref{fig:jetclass_0_skipwz_up},\protect\subref{fig:jetclass_0_std_skipwz_up} logarithmic 2D histogram of maximum probability versus uncertainty for, respectively, skipwz JetClass EDL $\lambda_t (0) $ without and with D-STD uncertainty.
    }
    \label{fig:jetclass_skipwz}
\end{figure}


The skiptwz models classify both top quark and boson as anomalous jets, so they have features from both skiptop and skipwz models. In Table~\ref{tab:JetClass}, the accuracy of skiptwz EDL models decreases as $\zeta$ increases similarly to the skiptop EDL models. The best performing model is still the EDL $\lambda_t (0)$ model with D-STD uncertainty, and networks with non-zero $\zeta$ have slightly lower AUROC and AUROC-STD. Again, D-STD uncertainty either is negligible or decreases the performance with a lower AUROC-STD compared to AUROC. In Figure~\ref{fig:jetclass_skiptwz}(a)-(b), the OOD jet $t \to b \ell v$ is often predicted as $H \to \ell v q q'$ with low uncertainties due to $H \to \ell v q q'$ being the only ID jet containing a lepton. As a result, the OOD uncertainty distributions in  Figure~\ref{fig:jetclass_skiptwz}(c)-(f) are often bimodal with low uncertainty $t \to b \ell v$ and other high uncertainty OOD jets. Again, D-STD improves the performance only for EDL $\lambda_t (0)$ because it increases the range of uncertainties and the OOD uncertainties tend to be more spread out as opposed to ID uncertainties, which increases the AUROC in Figure~\ref{fig:jetclass_skiptwz}(g)-(j). For non-zero $\zeta$, D-STD uncertainty seems to put more OOD and ID jets near the middle uncertainty rather than at the ends, which worsens the performance.


\begin{figure}[!h]

\centering
    
    \subfloat[]{
    \includegraphics[width=0.5\textwidth]{figures/jetclass/skiptwz/1.0/labels_preds_unc_total.pdf}
    \label{fig:jetclass_1.0_skiptwz_lpu}
    }
    \subfloat[]{
    \includegraphics[width=0.5\textwidth]{figures/jetclass/skiptwz/1.0_std/labels_preds_unc_total.pdf}
    \label{fig:jetclass_1.0_std_skiptwz_lpu}
    }
% 0.23, 0.27

    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiptwz/1.0/unc_separate_log.pdf}
        \label{fig:jetclass_1.0_skiptwz_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiptwz/1.0/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_1.0_skiptwz_up}
    }
    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiptwz/1.0_std/unc_separate_log.pdf}
        \label{fig:jetclass_1.0_std_skiptwz_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiptwz/1.0_std/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_1.0_std_skiptwz_up}
    }

    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiptwz/0/unc_separate_log.pdf}
        \label{fig:jetclass_0_skiptwz_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiptwz/0/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_0_skiptwz_up}
    }
    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiptwz/0_std/unc_separate_log.pdf}
        \label{fig:jetclass_0_std_skiptwz_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiptwz/0_std/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_0_std_skiptwz_up}
    }
    
    
    \caption{\protect\subref{fig:jetclass_1.0_skiptwz_lpu},\protect\subref{fig:jetclass_1.0_std_skiptwz_lpu} 2D histogram of the predicted label plus the uncertainty versus label, \protect\subref{fig:jetclass_1.0_skiptwz_us},\protect\subref{fig:jetclass_1.0_std_skiptwz_us} uncertainty distribution, separated by correctly and incorrectly classified jets, and \protect\subref{fig:jetclass_1.0_skiptwz_up},\protect\subref{fig:jetclass_1.0_std_skiptwz_up} logarithmic 2D histogram of maximum probability versus uncertainty for, respectively, skiptwz JetClass EDL $\lambda_t (1.0) $ without and with D-STD uncertainty.
    \protect\subref{fig:jetclass_0_skiptwz_us},\protect\subref{fig:jetclass_0_std_skiptwz_us} uncertainty distribution, separated by correctly and incorrectly classified jets, and \protect\subref{fig:jetclass_0_skiptwz_up},\protect\subref{fig:jetclass_0_std_skiptwz_up} logarithmic 2D histogram of maximum probability versus uncertainty for, respectively, skiptwz JetClass EDL $\lambda_t (0) $ without and with D-STD uncertainty.
    }
    \label{fig:jetclass_skiptwz}
\end{figure}

The skiph models treats Higgs boson jets as OOD. Unlike the other anomaly detection models, the EDL $\lambda_t (0)$ without D-STD uncertainty has the highest AUROC. In this case, D-STD actually worsens the performance for all EDL models, especially for EDL $\lambda_t (0)$. In Figure~\ref{fig:jetclass_skiph}(a)-(b), the OOD jet $H \to \ell v q q'$ is often predicted as $t \to b \ell v$ with low uncertainties due to the same reason of $t \to b \ell v$ being the only ID jet containing a lepton. This causes a large number of OOD jets to be lower uncertainties in Figure~\ref{fig:jetclass_skiph}(c)-(f). A surprising aspect is that D-STD uncertainty lowers the AUROC for EDl $\lambda_t (0)$, and it can be analyzed in Figure~\ref{fig:jetclass_skiph}(g)-(j). It seems that \todo{I don't know why D-STD does this}{}

\begin{figure}[!h]

\centering
    
    \subfloat[]{
    \includegraphics[width=0.5\textwidth]{figures/jetclass/skiph/1.0/labels_preds_unc_total.pdf}
    \label{fig:jetclass_1.0_skiph_lpu}
    }
    \subfloat[]{
    \includegraphics[width=0.5\textwidth]{figures/jetclass/skiph/1.0_std/labels_preds_unc_total.pdf}
    \label{fig:jetclass_1.0_std_skiph_lpu}
    }
% 0.23, 0.27

    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiph/1.0/unc_separate_log.pdf}
        \label{fig:jetclass_1.0_skiph_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiph/1.0/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_1.0_skiph_up}
    }
    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiph/1.0_std/unc_separate_log.pdf}
        \label{fig:jetclass_1.0_std_skiph_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiph/1.0_std/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_1.0_std_skiph_up}
    }

    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiph/0/unc_separate_log.pdf}
        \label{fig:jetclass_0_skiph_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiph/0/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_0_skiph_up}
    }
    \subfloat[]{
        \includegraphics[width=0.2185\textwidth]{figures/jetclass/skiph/0_std/unc_separate_log.pdf}
        \label{fig:jetclass_0_std_skiph_us}
    }
    \subfloat[]{
        \raisebox{-0.15cm}{
        \includegraphics[width=0.2565\textwidth]{figures/jetclass/skiph/0_std/unc_prob_total_log.pdf}
        }
        \label{fig:jetclass_0_std_skiph_up}
    }
    
    
    \caption{\protect\subref{fig:jetclass_1.0_skiph_lpu},\protect\subref{fig:jetclass_1.0_std_skiph_lpu} 2D histogram of the predicted label plus the uncertainty versus label, \protect\subref{fig:jetclass_1.0_skiph_us},\protect\subref{fig:jetclass_1.0_std_skiph_us} uncertainty distribution, separated by correctly and incorrectly classified jets, and \protect\subref{fig:jetclass_1.0_skiph_up},\protect\subref{fig:jetclass_1.0_std_skiph_up} logarithmic 2D histogram of maximum probability versus uncertainty for, respectively, skiph JetClass EDL $\lambda_t (1.0) $ without and with D-STD uncertainty.
    \protect\subref{fig:jetclass_0_skiph_us},\protect\subref{fig:jetclass_0_std_skiph_us} uncertainty distribution, separated by correctly and incorrectly classified jets, and \protect\subref{fig:jetclass_0_skiph_up},\protect\subref{fig:jetclass_0_std_skiph_up} logarithmic 2D histogram of maximum probability versus uncertainty for, respectively, skiph JetClass EDL $\lambda_t (0) $ without and with D-STD uncertainty.
    }
    \label{fig:jetclass_skiph}
\end{figure}
